Synthesis and electronic properties of Nd$_{n+1}$Ni$_{n}$O$_{3n+1}$ Ruddlesden-Popper nickelate thin films

The rare-earth nickelates possess a diverse set of collective phenomena including metal-to-insulator transitions, magnetic phase transitions, and, upon chemical reduction, superconductivity. Here, we demonstrate epitaxial stabilization of layered nickelates in the Ruddlesden-Popper form, Nd$_{n+1}$Ni$_n$O$_{3n+1}$, using molecular beam epitaxy. By optimizing the stoichiometry of the parent perovskite NdNiO$_3$, we can reproducibly synthesize the $n = 1 - 5$ member compounds. X-ray absorption spectroscopy at the O $K$ and Ni $L$ edges indicate systematic changes in both the nickel-oxygen hybridization level and nominal nickel filling from 3$d^8$ to 3$d^7$ as we move across the series from $n = 1$ to $n = \infty$. The $n = 3 - 5$ compounds exhibit weakly hysteretic metal-to-insulator transitions with transition temperatures that depress with increasing order toward NdNiO$_3$ ($n = \infty)$.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
